Assessing dengue fever risk in Costa Rica by using climate variables and machine learning techniques

Dengue fever is a vector-borne disease mostly endemic to tropical and subtropical countries that affect millions every year and is considered a significant burden for public health. Its geographic distribution makes it highly sensitive to climate conditions. Here, we explore the effect of climate variables using the Generalized Additive Model for location, scale, and shape (GAMLSS) and Random Forest (RF) machine learning algorithms. Using the reported number of dengue cases, we obtained reliable predictions. The uncertainty of the predictions was also measured. These predictions will serve as input to health officials to further improve and optimize the allocation of resources prior to dengue outbreaks.

==> name.tex <==
Dengue constitutes a significant public health problem in Costa Rica, a tropical country with multiple microclimates separated by short distances, ideal for the proliferation of mosquitoes and challenging territory for surveillance. Resources for dengue prevention in the country are limited. Therefore, it becomes valuable to have tools that predict the places with the highest risk of having an outbreak in periods that allow timely responses by decision-makers.

The importance of climate information regarding dengue fever incidence has been well established\cite{}. Here, we incorporated climate information to predict the relative risk of dengue in 32 different cantons in Costa Rica using GAMLSS and RF models 

The dynamics of dengue incidence change geographically and temporally, so more localized studies may be necessary and explore different methodologies to find what works well in which situations. Here, we propose a GMALSS and a RF method which showed well performance


In a first approach \cite{}, we implemented a Generalized Additive model and a Randon Forest, which performed well predicting the relative risk of dengue in five of the 32 cantons used in this study. However, the model's efficacy and predictions were limited by the availability and quality of meteorological data. In addition, knowing the climatic covariates was a necessary condition to predict dengue behavior. In this new result, these limitations were overcome using satellite information and proposing a vector auto-regressive (VAR) model to obtain climate predictions shortly, which are incorporated in the models to forecast the relative risk.   

Our results showed that using data from 2000-2020 to tren the models, the vector autoregressive model performs well-predicting climatic variables, and the GAMLSS and the Random Forest model successfully predict dengue relative risk in the first three months of 2021, corresponding to the testing period.

 We have used a set of common climate variables in our analysis, considering additional climate covariates could provide additional information or benefits in predictive accuracy. Numerous studies have shown correlations between dengue cases and temperature, relative humidity, and precipitation as indicated in the introduction as well as absolute humidity, more recently5

Understanding how Ae. aegypti mosquitoes respond to climate conditions is crucial for developing climate-based early warning systems for dengue prediction.  
